First measurements of remoTES cryogenic calorimeters: easy-to-fabricate particle detectors for a wide choice of target materials

Low-temperature calorimeters based on a readout via Transition Edge Sensors (TESs) and operated below $100$ mK are well suited for rare event searches with outstanding resolution and low thresholds. We present first experimental results from two detector prototypes using a novel design of the thermometer coupling denoted remoTES, which further extends the applicability of the TES technology by including a wider class of potential absorber materials. In particular, this design facilitates the use of materials whose physical and chemical properties, as e.g. hygroscopicity, low hardness and low melting point, prevent the direct fabrication of the TES onto their surface. This is especially relevant in the context of the COSINUS experiment (Cryogenic Observatory for SIgnals seen in Next-Generation Underground Searches), where sodium iodide (NaI) is used as absorber material. With two remoTES prototype detectors operated in an above-ground R&D facility, we achieve energy resolutions of $\sigma=87.8$ eV for a $2.33$ g silicon absorber and $\sigma = 193.5$ eV for a $2.27$ g $\alpha$-TeO$_{2}$ absorber, respectively. RemoTES calorimeters offer - besides the wider choice of absorber materials - a simpler production process combined with a higher reproducibility for large detector arrays and an enhanced radiopurity standard.

==> RemoTES(Version6018)/authors.tex <==
%copied from COSINUS wiki, version 08/31/2021

%%% AUTHORS %%%

\author[1]{G.~Angloher}
\author[1]{M.R.~Bharadwaj}
\author[2]{I.~Dafinei}
\author[3,4]{N.~Di~Marco}
\author[5,7]{L.~Einfalt}
\author[2, 3]{F.~Ferroni}
\author[5]{ S.~Fichtinger}
\author[4,6]{A.~Filipponi}
\author[1]{T.~Frank}
\author[5]{M.~Friedl}
\author[5,7]{ A.~Fuss}
\author[8]{Z.~Ge}
\author[9]{M.~Heikinheimo}
\author[9]{K.~Huitu}
\author[1]{M.~Kellermann}
\author[5,7]{R.~Maji}
\author[1]{M.~Mancuso}
\author[3,4]{L.~Pagnanini}
\author[1]{F.~Petricca}
\author[4]{S.~Pirro}
\author[1]{F.~Pr\"obst}
\author[4,6]{G.~Profeta}
\author[3,4]{A.~Puiu}
\author[5,7]{F.~Reindl}
\author[1]{K.~Sch\"affner}
\author[5,7]{J.~Schieck}
\author[5,7]{D.~Schmiedmayer}
\author[5,7]{C.~Schwertner}
\author[1]{M.~Stahlberg}
\author[9]{A.~Stendahl}
\author[5]{F.~Wagner}
\author[8]{S.~Yue}
\author[1]{V.~Zema}
\author[8]{Y.~Zhu}
\author[]{(The COSINUS collaboration)}+



%\author[ ]{\\
%  (The COSINUS Collaboration)
%}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Corresponding Authors 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\thankstext{te1}{Corresponding author: \href{mailto:<email_address>}{mailto:<email_address>}}
%\thankstext{te2}{Corresponding author: \href{mailto:<email_address>}{mailto:<email_address>}}
%\affil[*]{Corresponding author: some.name@mymail.com}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % AFFILIATIONS 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\affil[1]{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}
\affil[2]{INFN - Sezione di Roma, 00185 Roma - Italy}
\affil[3]{Gran Sasso Science Institute, 67100 L'Aquila - Italy}
\affil[4]{INFN - Laboratori Nazionali del Gran Sasso, 67010 Assergi}
\affil[5]{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}
\affil[6]{Dipartimento di Scienze Fisiche e Chimiche, Universit\`a degli Studi dell'Aquila, 67100 L'Aquila - Italy}
\affil[7]{Atominstitut, Technische Universit\"at Wien, 1020 Wien - Austria}
\affil[8]{SICCAS - Shanghai Institute of Ceramics, Shanghai - P.R.China 200050}
\affil[9]{Helsinki Institute of Physics, 00560 Helsinki - Finland}


==> RemoTES(Version6018)/authors_new.tex <==
%%% AUTHORS %%%
\author{G.~Angloher}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}

\author{M.R.~Bharadwaj}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}

\author{I.~Dafinei}
\affiliation{INFN - Sezione di Roma, 00185 Roma - Italy}

\author{N.~Di~Marco}
\affiliation{Gran Sasso Science Institute, 67100 L'Aquila - Italy}
\affiliation{INFN - Laboratori Nazionali del Gran Sasso, 67010 Assergi - Italy}

\author{L.~Einfalt}
\affiliation{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}
\affiliation{Atominstitut, Technische Universit\"at Wien, 1020 Wien - Austria}

\author{F.~Ferroni}
\affiliation{Gran Sasso Science Institute, 67100 L'Aquila - Italy}
\affiliation{INFN - Sezione di Roma, 00185 Roma - Italy}

\author{S.~Fichtinger}
\affiliation{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}

\author{A.~Filipponi}
\affiliation{Dipartimento di Scienze Fisiche e Chimiche, Universit\`a degli Studi dell'Aquila, 67100 L'Aquila - Italy}
\affiliation{INFN - Laboratori Nazionali del Gran Sasso, 67010 Assergi - Italy}

\author{T.~Frank}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}

\author{M.~Friedl}
\affiliation{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}

\author{A.~Fuss}
\affiliation{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}
\affiliation{Atominstitut, Technische Universit\"at Wien, 1020 Wien - Austria}

\author{Z.~Ge}
\affiliation{SICCAS - Shanghai Institute of Ceramics, Shanghai - P.R.China 200050}

\author{M.~Heikinheimo}
\affiliation{Helsinki Institute of Physics, Univ. of Helsinki, 00014 Helsinki - Finland}

\author{K.~Huitu}
\affiliation{Helsinki Institute of Physics, Univ. of Helsinki, 00014 Helsinki - Finland}

\author{M.~Kellermann}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}

\author{R.~Maji}
\affiliation{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}
\affiliation{Atominstitut, Technische Universit\"at Wien, 1020 Wien - Austria}

\author{M.~Mancuso}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}

\author{L.~Pagnanini}
\affiliation{Gran Sasso Science Institute, 67100 L'Aquila - Italy}
\affiliation{INFN - Laboratori Nazionali del Gran Sasso, 67010 Assergi - Italy}

\author{F.~Petricca}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}

\author{S.~Pirro}
\affiliation{INFN - Laboratori Nazionali del Gran Sasso, 67010 Assergi - Italy}

\author{F.~Pr\"obst}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}

\author{G.~Profeta}
\affiliation{Dipartimento di Scienze Fisiche e Chimiche, Universit\`a degli Studi dell'Aquila, 67100 L'Aquila - Italy}
\affiliation{INFN - Laboratori Nazionali del Gran Sasso, 67010 Assergi - Italy} 

\author{A.~Puiu}
\affiliation{Gran Sasso Science Institute, 67100 L'Aquila - Italy}
\affiliation{INFN - Laboratori Nazionali del Gran Sasso, 67010 Assergi - Italy}

\author{F.~Reindl}
\email{Corresponding author, florian.reindl@tuwien.ac.at}
\affiliation{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}
\affiliation{Atominstitut, Technische Universit\"at Wien, 1020 Wien - Austria}

\author{K.~Sch\"affner}
\email{Corresponding author, karoline.schaeffner@mpp.mpg.de}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}

\author{J.~Schieck}
\affiliation{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}
\affiliation{Atominstitut, Technische Universit\"at Wien, 1020 Wien - Austria}

\author{D.~Schmiedmayer}
\affiliation{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}
\affiliation{Atominstitut, Technische Universit\"at Wien, 1020 Wien - Austria}

\author{C.~Schwertner}
\affiliation{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}
\affiliation{Atominstitut, Technische Universit\"at Wien, 1020 Wien - Austria}

\author{M.~Stahlberg}
\email{Corresponding author, martin.stahlberg@mpp.mpg.de}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}

\author{A.~Stendahl}
\affiliation{Helsinki Institute of Physics, Univ. of Helsinki, 00014 Helsinki - Finland}

\author{F.~Wagner}
\affiliation{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}

\author{S.~Yue}
\affiliation{SICCAS - Shanghai Institute of Ceramics, Shanghai - P.R.China 200050}

\author{V.~Zema}
\email{Corresponding author, 
vanezema@mpp.mpg.de}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}

\author{Y.~Zhu}
\affiliation{SICCAS - Shanghai Institute of Ceramics, Shanghai - P.R.China 200050}

\collaboration{The COSINUS Collaboration}
\author{A.~Bento}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}
\affiliation{LIBPhys-UC, Physics Departments, University of Coimbra, 3004-516 Coimbra - Portugal}
\author{L.~Canonica}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}
\author{A.~Garai}
\affiliation{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}



==> authors.tex <==
%copied from COSINUS wiki, version 08/31/2021

%%% AUTHORS %%%

\author[1]{G.~Angloher}
\author[1]{M.R.~Bharadwaj}
\author[2]{I.~Dafinei}
\author[3,4]{N.~Di~Marco}
\author[5,7]{L.~Einfalt}
\author[2, 3]{F.~Ferroni}
\author[5]{ S.~Fichtinger}
\author[4,6]{A.~Filipponi}
\author[1]{T.~Frank}
\author[5]{M.~Friedl}
\author[5,7]{ A.~Fuss}
\author[8]{Z.~Ge}
\author[9]{M.~Heikinheimo}
\author[9]{K.~Huitu}
\author[1]{M.~Kellermann}
\author[5,7]{R.~Maji}
\author[1]{M.~Mancuso}
\author[3,4]{L.~Pagnanini}
\author[1]{F.~Petricca}
\author[4]{S.~Pirro}
\author[1]{F.~Pr\"obst}
\author[4,6]{G.~Profeta}
\author[3,4]{A.~Puiu}
\author[5,7]{F.~Reindl}
\author[1]{K.~Sch\"affner}
\author[5,7]{J.~Schieck}
\author[5,7]{D.~Schmiedmayer}
\author[5,7]{C.~Schwertner}
\author[1]{M.~Stahlberg}
\author[9]{A.~Stendahl}
\author[5]{F.~Wagner}
\author[8]{S.~Yue}
\author[1]{V.~Zema}
\author[8]{Y.~Zhu}
\author[]{(The COSINUS collaboration)}+



%\author[ ]{\\
%  (The COSINUS Collaboration)
%}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Corresponding Authors 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\thankstext{te1}{Corresponding author: \href{mailto:<email_address>}{mailto:<email_address>}}
%\thankstext{te2}{Corresponding author: \href{mailto:<email_address>}{mailto:<email_address>}}
%\affil[*]{Corresponding author: some.name@mymail.com}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % AFFILIATIONS 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\affil[1]{Max-Planck-Institut f\"ur Physik, 80805 M\"unchen - Germany}
\affil[2]{INFN - Sezione di Roma, 00185 Roma - Italy}
\affil[3]{Gran Sasso Science Institute, 67100 L'Aquila - Italy}
\affil[4]{INFN - Laboratori Nazionali del Gran Sasso, 67010 Assergi}
\affil[5]{Institut f\"ur Hochenergiephysik der \"Osterreichischen Akademie der Wissenschaften, 1050 Wien - Austria}
\affil[6]{Dipartimento di Scienze Fisiche e Chimiche, Universit\`a degli Studi dell'Aquila, 67100 L'Aquila - Italy}
\affil[7]{Atominstitut, Technische Universit\"at Wien, 1020 Wien - Austria}
\affil[8]{SICCAS - Shanghai Institute of Ceramics, Shanghai - P.R.China 200050}
\affil[9]{Helsinki Institute of Physics, 00560 Helsinki - Finland}

